SimMIL: A Universal Weakly Supervised Pre-Training Framework for Multi-Instance Learning in Whole Slide Pathology Images

Various multi-instance learning (MIL) based approaches have been developed and successfully applied to whole-slide pathological images (WSI). Existing MIL methods emphasize the importance of feature aggregators, but largely neglect the instance-level representation learning. They assume that the availability of a pre-trained feature extractor can be directly utilized or fine-tuned, which is not always the case. This paper proposes to pre-train feature extractor for MIL via a weakly-supervised scheme, i.e., propagating the weak bag-level labels to the corresponding instances for supervised learning. To learn effective features for MIL, we further delve into several key components, including strong data augmentation, a non-linear prediction head and the robust loss function. We conduct experiments on common large-scale WSI datasets and find it achieves better performance than other pre-training schemes (e.g., ImageNet pre-training and self-supervised learning) in different downstream tasks. We further show the compatibility and scalability of the proposed scheme by deploying it in fine-tuning the pathological-specific models and pre-training on merged multiple datasets. To our knowledge, this is the first work focusing on the representation learning for MIL.

==> tabs/tab1.tex <==
\begin{table}[h!]{
    \caption{Preliminary results (\%) of instance-level linear probing (Acc-LP) and fine-tuning (Acc-FT) and weakly supervised bag classification with max/mean pooling aggregator (Max-/Mean-AUC). 
    % with feature extractors using different pre-training schemes. denotes AUC (\%) achieved by 
    }
    \label{results_on_NCTCRC}
    % \resizebox{1\linewidth}{!}
    {
    \centering
    \begin{center}
    \begin{tabular}{lcccc}
    \hline
    \multirow{2}{*}{\textbf{\makecell{Scheme}}}  &  
     \multicolumn{2}{c}{ NCTCRC} &
    \multicolumn{2}{c}{ NCTCRC-BAGS} \\
     % \cmidrule(lr){2-3}  \cmidrule(lr){4-5} 
     & Acc-LP& Acc-FT  & Max-AUC  & Mean-AUC \\
    \hline 
     ImageNet & 88.66 & 93.71 & 90.60 & 96.64 \\
     MoCo v2 & \textbf{92.14} & 94.45 & 97.46 & 93.67 \\
     SimCLR  & 91.41 & \textbf{94.62} & 98.37 & 95.39  \\
     % SimMIL (Ours) & 73.96&? & \textbf{99.78} & \textbf{96.29} \\
     SimpleMIL & 74.73 & 88.84 &  \textbf{99.04} & \textbf{98.53} \\
     \hline
    \end{tabular}
    \end{center}
    }
    }
\end{table}

==> tabs/tabA6.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{ccc}
        \toprule    
        \multirow{2}{*}{Assumption}  & \multicolumn{2}{c}{Number of positive / negative bags} \\
        \cmidrule(lr){2-3}
        & Train & Test \\
        \midrule
        Standard & 1030 / 957 & 88 / 51 \\
        \bottomrule
    \end{tabular}
\caption{The summary of the created NCTCRC-BAGS dataset under MIL assumptions with number of positive and negative bags in training and test sets.}
\label{NCTCRC-Sumary}
\end{table}

==> tabs/tabB7.tex <==
\begin{table}[ht!]
    \centering
    \resizebox{\linewidth}{!}
    {
    \begin{tabular}{ccccccccc}
    \toprule
    \multirow{2}{*}{\textbf{Agg.}} & 
    \multirow{2}{*}{\textbf{Method}} &
    \multirow{2}{*}{\textbf{Arch.}} &
    \multicolumn{2}{c}{Camelyon16} & \multicolumn{2}{c}{TCGA-NSCLC} & \multicolumn{2}{c}{TCGA-BRCA} \\
    % \cline{4-9}
    \cmidrule(lr){4-5}  \cmidrule(lr){6-7} 
    \cmidrule(lr){8-9}  
     &  &  & Acc & AUC & Acc & AUC & Acc & AUC \\ 
     \midrule
    \multirow{4}{*}{\makecell{Max \\ Pooling}} & MoCo V2 & ResNet50 
    & 70.54 & \underline{74.13} & 89.52 & 95.28 & 66.67 & 75.26 \\
    & SwAV & ResNet50 & \underline{73.64} & 69.03 & \underline{89.52} & \underline{96.64} & 78.79 & 85.37 \\
    & SimMIL\footnotesize{(ours)} & ResNet18 & \textbf{80.62} & \textbf{79.63} & 89.52 & 95,91 & \textbf{87.88} & \underline{91.02} \\
    & SimMIL\footnotesize{(ours)} & ResNet50 & 72.87 & 65.23 & \textbf{90.48} & \textbf{97.45} & \underline{87.27} & \textbf{93.44} \\
    \midrule
    \multirow{4}{*}{\makecell{Mean \\ Pooling}} & MoCo V2 & ResNet50 & 65.89 & \underline{58.21} & 80.48 & 87.00 & 63.64 & 72.61 \\
    & SwAV & ResNet50 & 68.22 & 53.00 & \underline{87.14} & \underline{93.76} & 80.00 & 81.86 \\
    & SimMIL\footnotesize{(ours)} & ResNet18 & \textbf{75.19} & \textbf{59.48} & 86.67 & 92.86 & \underline{84.85} & \underline{87.59} \\
    & SimMIL\footnotesize{(ours)} & ResNet50 & \underline{70.54} & 57.28 & \textbf{89.52} & \textbf{95.43} & \textbf{90.30} & \textbf{90.35} \\
    \bottomrule
    \end{tabular}
    }
    \caption{Results (\%) of scaling experiments on model size, comparing ResNet18 and ResNet50. Acc and AUC are reported.}
    \label{ablation_backbone}
\end{table}

==> tabs/tabC8.tex <==
\begin{table}[ht!]
    \centering
    \resizebox{\linewidth}{!}
    {
    \begin{tabular}{ccccccccc}
    \toprule
    \multirow{2}{*}{\textbf{Agg.}} & 
    \multirow{2}{*}{\textbf{Method}} &
    \multirow{2}{*}{\textbf{Arch.}} &
    \multicolumn{2}{c}{Camelyon16} & \multicolumn{2}{c}{TCGA-NSCLC} & \multicolumn{2}{c}{TCGA-BRCA} \\
    % \cline{4-9}
    \cmidrule(lr){4-5}  \cmidrule(lr){6-7} 
    \cmidrule(lr){8-9}  
     &  &  & Acc & AUC & Acc & AUC & Acc & AUC \\ 
     \midrule
    \multirow{6}{*}{\makecell{TransMIL}} & ImageNet & ResNet18 
    & 76.74 & 74.78 & 82.38 & 88.91 & \textbf{84.24} & 85.58 \\
    & MoCo V2 & ResNet18  & 80.62 & 75.13 & \underline{90.48} & 94.60 & 74.55 & 76.79 \\
    & SimCLR & ResNet18 & 75.19 & 71.29 & 88.57 & 91.68 & 76.36 & 79.89 \\
    & CLIP & ResNet50  & 75.19 & 69.11 & 84.29 & 91.38 & 82.42 & \textbf{90.40} \\
    & SRCL & CTransPath  & \textbf{86.05} & \textbf{87.35} & 89.05 & \underline{96.04} & 80.61 & \underline{89.60} \\
    & SimMIL\footnotesize{(ours)} & ResNet18  & \underline{81.40} & \underline{79.95} & \textbf{94.76} & \textbf{97.18} & \underline{82.42} & 83.37 \\
    \midrule
    \multirow{6}{*}{\makecell{DTFD-MIL}} & ImageNet & ResNet18 & 84.50 & 83.90 & 88.10 & 92.10 & 71.52 & 80.59 \\
    & MoCo V2 & ResNet18 & 54.26 & 55.99 & 77.62 & 86.24 & 74.55 & 74.86 \\
    & SimCLR & ResNet18 & 78.29 & 81.56 & 87.62 & 93.44 & 82.42 & 85.70 \\
    & CLIP & ResNet50  & 67.44 & 56.32 & 71.90 & 76.96 & 58.18 & 67.17 \\
    & SRCL & CTransPath  & \textbf{93.80} & \textbf{95.58} & \underline{90.00} & \underline{96.46} & \underline{89.70} & \textbf{93.72} \\
    & SimMIL\footnotesize{(ours)} & ResNet18 & \underline{93.02} & \underline{91.10} & \textbf{94.29} & \textbf{97.58} & \textbf{90.30} & \underline{92.48} \\
    \bottomrule
    \end{tabular}
    }
    \caption{Results (\%) of bag classification using TransMIL and DTFD-MIL as aggretators. Acc and AUC are reported.}
    \label{additional_results}
\end{table}

==> tabs/tabD9.tex <==
\begin{table}[ht!]
    \centering
    \begin{tabular}{cccc}
        \toprule    
        Aggregator  & Scheduler & LR & weight decay \\
        \midrule
        Max Pooling & Adam & $1\times10^{-4}$ & $1\times10^{-4}$ \\
        Mean Pooling & Adam & $1\times10^{-4}$ & $1\times10^{-4}$ \\
        ABMIL & Adam & $1\times10^{-4}$ & $1\times10^{-4}$ \\
        DSMIL & Adam & $1\times10^{-4}$ & $1\times10^{-4}$ \\
        CLAM-SB & Adam & $1\times10^{-4}$ & $1\times10^{-5}$ \\
        % TransMIL & Adam & $2\times10^{-4}$ & $1\times10^{-5}$ \\
        % DTFD-MIL & MultiStep & $1\times10^{-4}$  & $5\times10^{-3}$\\
        \bottomrule
    \end{tabular}
\caption{The summary of the hyper-parameters using in the training of different aggreation networks.}
\label{aggregation_param}
\end{table}
